Scissorhands: Exploiting the Persistence of Importance Hypothesis for LLM KV Cache Compression at Test Time

Large language models(LLMs) have sparked a new wave of exciting AI applications. Hosting these models at scale requires significant memory resources. One crucial memory bottleneck for the deployment stems from the context window. It is commonly recognized that model weights are memory hungry; however, the size of key-value embedding stored during the generation process (KV cache) can easily surpass the model size. The enormous size of the KV cache puts constraints on the inference batch size, which is crucial for high throughput inference workload. Inspired by an interesting observation of the attention scores, we hypothesize the persistence of importance: only pivotal tokens, which had a substantial influence at one step, will significantly influence future generations. Based on our empirical verification and theoretical analysis around this hypothesis, we propose Scissorhands, a system that maintains the memory usage of the KV cache at a fixed budget without finetuning the model. In essence, Scissorhands manages the KV cache by storing the pivotal tokens with a higher probability. We validate that Scissorhands reduces the inference memory usage of the KV cache by up to 5X without compromising model quality. We further demonstrate that Scissorhands can be combined with 4-bit quantization, traditionally used to compress model weights, to achieve up to 20X compression.

==> 04_method_old.tex <==
\section{Sequential token generation under budget} 
\label{sec:method}
%The above hypothesis and observation provide insights for understanding the behavior of LLMs. At the same time, it suggests a new opportunity to reduce KV cache memory. In this section, we present our method \name{}, which exploits the above observation to reduce KV cache memory. In Section~\ref{sec:method_sample}, we present the detailed sampling scheme that accurately approximates the attention outputs for a future generation step. 


In this section, we present our proposal \name{}, which reduces the KV cache memory from the sequence length dimension without fine-tuning the model. In Section~\ref{sec:method_sample}, we present the sampling algorithm \name{} uses to maintain the KV cache under a given budget $B$. Section~\ref{sec:method_theory} provides a theoretical analysis of the sampling strategy and the approximate error.



\subsection{Budgeted sample for single attention head}
\label{sec:method_sample}
In this section, for the sake of the discussion, we drop the layer number notation $i$ and batch size dimension.  $\mathcal{K}_t, \mathcal{V}_t \in  R^{t \times d}$ denote for the KV cache until step $t$. $x_t\in\R^{1\times d}$ is a row vector denotes for the input to attention at step $t$.

The output of a single attention head at step $t$ can be written as,
\begin{equation}
    a_{t} = \sum_{i=1}^{t} \alpha_{t,i} \mathcal{V}[i]_t  \textrm{ where } \alpha_{t, i} = \frac{\exp(\langle  x_t W_K , \mathcal{K}_t[i] \rangle )}{\sum_{i=1}^{t} \exp(\langle  x_t W_K , \mathcal{K}_t[i] \rangle )} \label{eq:gen}
\end{equation}

%\textbf{Intuition}
\textbf{Intuition.} As shown in Section \ref{sec:hypos}, the attention scores $\alpha_{t,i}$ follow a strong power-law distribution. For the autoregressive generation process, if there exists an oracle such that we can identify the heavy score tokens before the future generation step, then the memory of the KV cache can be significantly reduced by only storing the heavy score tokens. Fortunately, the \hypothesis{} provides us with such an oracle. It states that only historical tokens with significant contributions toward generated tokens will have significant contributions toward future tokens. 

\textbf{Challenges.} LLMs are deployed on hardware with a fixed memory. To meet the hard requirement, the algorithm should maintain the cache at fixed memory. Second, LLMs are already computationally intensive. The sampling algorithm should be efficient to avoid an extra burden on computation. 

Given a fixed memory budget for one attention head to be $N$ tokens. In other words, we are allowed to store key and value embedding for $N$ previous tokens. We describe the problem as follows,

\begin{definition}[Sequential generation at an attention-head under budget $N$]
    Given a prompt containing $p$ tokens and their input to the head as $\{x_1, \ldots, x_p\}$, a stream of generate token embeddings at previous layers and their input to the head as $\{x_{p+1}, ... x_t, ...\}$, the problem of sequential generation at an attention head under budget $N$ is to maintain a set of token ids $S_t$ at every generation step $t$ with $|S_t| \leq N$. Only the key and value for the tokens in $S_t$ are stored, i.e $ \Bar{\mathcal{K}}_t = \{\mathcal{K}_t[i] \; | \; i \in S_t \}$ and $\Bar{\mathcal{V}}_t = \{\mathcal{V}_t[i] \; | \; i \in S_t \}$ and estimate attention output as Equation~\ref{eq:gen} with only $\Bar{\mathcal{K}}_t, \Bar{\mathcal{V}}_t $. 
\end{definition}

% \begin{definition}[Sequential generation at an attention-head under budget $n$]
%     Given a prompt containing $p$ tokens and their input to the head as $\{x_1, \ldots, x_p\}$, a stream of generate token embeddings at previous layers and their input to the head as $\{x_{p+1}, ... x_t, ...\}$, the problem of sequential token generation at an attention head under budget $n$ is to maintain a set of token ids $S_t$ at all token positions $t$ of sequential generation, $|S_t| \leq n$ and KV cache only for $S_t$ , i.e $ \Bar{\mathcal{K}}_t = \{\mathcal{K}_t[i] \; | \; i \in S_t \}$ and $\Bar{\mathcal{V}}_t = \{\mathcal{V}_t[i] \; | \; i \in S_t \}$ and estimate equation \ref{eq:gen} at each $t > p$. 
% \end{definition}

% The problem of maintaining $n$ tokens from the given prompt tokens and stream of generated tokens seems related to reservoir sampling problem \cite{tille2006sampling}. If a oracle can correctly predict the $\alpha_{t, i}$ for all $i$ and if $\alpha_{t_1, i} = \alpha_{t_2, i}$ for all $t_1, t_2$, then exact solutions to obtain best sample for estimation of equation \ref{eq:gen} are known in literature in the form of weighted reservoir sampling \cite{chao1982general} with $\alpha$s as the weights. However, the problem at hand varies in two main aspects. Firstly, the weights associated with each token can change and thus are dynamic. Also, these dynamic weights are revealed only for tokens that are present in the sample and at token $t$.  \aditya{remove?}

\textbf{Approach.} Inspired by the textbook solution of reservoir sampling and Least Recent Usage cache replacement algorithm, \name{} reserves a fixed memory buffer for KV cache. When the buffer is full,  \name{} drops a stored but non-important token from the cache to clear memory for the most recent token. Naturally, attention scores are used as the indicators for importance.

% \textbf{Approach.} \name{} decides whether to keep a token's key and value embedding from two aspects: 1) position, and 2) importance. 
% \begin{enumerate}
    
%     \item Position: Our observation shows that more recent tokens in the context window are more likely to receive high attention scores. At the same time, textbook solution for managing system cache relies on recent usage. Thus, \name{} keeps the most recent $R$ tokens in the KV cache with hight probability.
%     \emma{Related Position with Importance to solve efficient sampling }
%     \item Importance: \hypothesis{} suggest that pivotal tokens are more likely to stay influential. Thus, \name{} keeps the pivotal tokens with a higher probability.
% \end{enumerate}
 
% We present our sampling algorithm in Algorithm~\ref{alg:sampling}. We explore the links to reservoir sampling and what can be achieved elaborately in appendix \ref{appendix:sampling}.

\input{algorithms/sampling_1}
\input{B_algorithm}
We present the main algorithm in Algorithm~\ref{alg:sampling}, which can be divided into two stages. 
\begin{enumerate}
    \item For the generation steps where $t \leq N$, \name{} keeps storing all the KV cache to fill up the memory budget.
    \item For the generation steps where $t > N$, \name{} keep the most recent $r$ tokens, indicating the removal of one previously stored token embedding. To achieve this, a probability distribution is created over tokens outside of the recent window using the classifical \textit{inclusion probability proportional to weights}. We give related algorithm in Appendix~\ref{appendix:sampling}. $Z_{ts}$, noted as $\pi(t, s)$, is created such that 
    $$\sum_{s \in S_{t-1} / \{t{-}r{+}1,..,t\}} \pi(t, s) = (n-r)$$
     A single token is selected with probability distribution $1 - \pi(t, s)$ and replaced with token $t$. Intuitively the token with the least contribution is chosen with a high probability of being replaced. Practically, such probability distribution is efficient to construct with basic operation using the attention scores.  
\end{enumerate}

With a sampled KV cache, attention output can be computed by the following estimator 

\begin{equation}
    \hat{a}_{t} = \sum_{s \in S_{t-1}} \hat{\alpha}_{t,s} \Bar{\mathcal{V}}_t[s]  \textrm{ where } \hat{\alpha}_{t, s} = \frac{\exp(\langle  x_t W_K , \Bar{\mathcal{K}}_{t-1}[s] \rangle )}{\sum_{s \in S_{t-1}} \exp(\langle  x_t W_K , \Bar{\mathcal{K}}_t[s] \rangle )}
\end{equation}
% Until the generation step $t$ where $t = n$, \name{} keeps storing all the KV cache to fill up the memory budget.  For the generation step where $t > n$, \name{} first always keep the most recent $R$ tokens in $S_t$, indicating this requires removing one stored token embedding.  A sampling distribution is created over these tokens using the standard \textit{inclusion probability proportional to weights} $Z_{ts}$, called $\pi(t, s)$, is created such that 
% $$\sum_{s \in S_{t-1} / \{t{-}r{+}1,..,t\}} \pi(t, s) = (n-r)$$ 


% that the previous $t-R$ token outside the recent window has to share a budget of $(N-R)$. 

% At a generation step $t$, \name{} keep the most recent $R$ tokens in $S_t$, indicating that the previous $t-R$ token outside the recent window has to share a budget of $(N-R)$.


% has to be distributed over the previous $t-R$ tokens. The sampling proceeds as follows. While $t<n$ we keep storing all the tokens in our sample as memory budget is not reached. When $t$ exceeds $n$, we choose to always keep the $t^{th}$ token as it is part of the recent window. However, this requires removal of one of the previously stored tokens in $S_{t-1}$ which are not part of recent window.  A sampling distribution is created over these tokens using the standard \textit{inclusion probability proportional to weights} $Z_{ts}$, called $\pi(t, s)$, is created such that 
% $$\sum_{s \in S_{t-1} / \{t{-}r{+}1,..,t\}} \pi(t, s) = (n-r)$$ 
% We then select a single token with probability distribution $1 - \pi(t, s)$ and replace it with token $t$. Intuitively the token with least contribution is chosen with high probability to be replaced. We give details on IPPS \cite{tille2006sampling} in appendix \ref{appendix:sampling}

%\textbf{Computing attention output:}

\textbf{Practical implementation}

\textbf{Allocating budgets across attention heads.} An LLM typically consists of $L$ transformer layers where each layer has $H$ heads. A total memory budget of $B$ has to be distributed over layers and heads. Within each transformer layer, the budget is distributed evenly across heads. Within the entire model, we distributed the budget according to Figure~\ref{figure:verification}. The rule of thumb is to allocate more budget to later layers to compensate for the lower persistence ratio.


\subsection{Theoretical Analysis.} 
\label{sec:method_theory}
We study how much the tokens generated by the sampled KV cache deviate from the tokens generated by the original transformer using our simplified model in (\ref{eq:basic_transformer}). Let $\{\tilde{x}_t\}_{t=0}^T$ denote the tokens generated by a one-layer transformer with sampled KV cache:
\begin{align*}
    \tilde{a}_{t+1} & = \softmax\paren{\frac{1}{t}\tilde{x}_t W_Q\tilde{\mathcal{K}}_t^\top}\tilde{\mathcal{V}}_t^\top W_O\\
    \tilde{x}_{t+1} & = \mathcal{F}\paren{\tilde{a}_{t+1}}
\end{align*}
Here $\mathcal{F}$ is as defined in (\ref{eq:basic_mlp}), $\tilde{\mathcal{K}}_t = \{\tilde{x}_iW_K:i\in S_t\setminus\{t\}\}$ and $\tilde{\mathcal{V}}_t = \{\tilde{x}_iW_V:i\in S_t\setminus\{t\}\}$. For reference purposes, let $\{x_t\}_{t=0}^T$ denote the tokens generated by a vanilla one-layer transformer defined in (\ref{eq:basic_transformer}). We will bound the difference $\norm{x_t - \tilde{x}_t}_2$. 
\begin{theorem}
    \label{theo:error_bound_main}
    Let $\lambda_1,\lambda_2$ denote the largest singular values of $W_1$ and $W_2$ in (\ref{eq:basic_mlp}). Let
    \[
        \beta_{t,j} = \frac{\exp\paren{\sfrac{1}{t}\cdot\tilde{x}_tW_QW_K^\top\tilde{x}_j^\top}}{\sum_{i=1}^{t-1}\exp\paren{\sfrac{1}{t}\cdot\tilde{x}_tW_QW_K^\top\tilde{x}_i^\top}}
    \]
    and assume that each $\beta_{t,j} = cv_{t,j}$, where $v_{t,j}$ are sampled from a power-law distribution with pdf $f(x) = c(x+b)^{-k}$. Suppose that $\lambda_V\lambda_O(1+ \lambda_1\lambda_2)(1 + \lambda_Q\lambda_K) \leq \frac{1}{2}$. Let $T_{\min}$ and $T_{\max}$ denote the starting and maximum sequence length, respectively. If for all $t\in[T_{\min}, T_{\max}]$, $S_t$ contains only tokes with at most the largest $B\cdot T_{\max}$ values of $\beta_{t,j}$, that is, $\left|S_t\right| = B\cdot T_{\max}$ and $\min_{j\in S_t}\beta_{t,j} \geq \max_{j\notin\hat{S}_t}\beta_{t,j}$, then for all $\epsilon\in(0,1)$, with probability at least $1 - T_{\max}\exp\paren{-\frac{\epsilon^2b^2(T_{\min}-1)}{(k-2)^2(u-b)^2}} - T_{\max}\exp\paren{-\frac{2(T_{\min}-1)(1-B)^2}{(1-\epsilon)^2}}$, the following error bound must hold for all $t\in [T_{\min}, T_{\max}]$
    \begin{equation}
        \label{eq:err_bound}
        \E{\norm{x_t - \tilde{x}_t}_2} \leq \frac{2.1(1-B)}{(1-\epsilon)^2}\paren{k -  (k-1)\paren{\frac{1-\epsilon}{B-\epsilon}}^{\frac{1}{k-1}}}
    \end{equation}
\end{theorem}
In Theorem \ref{theo:error_bound_main}, the definition of $\beta_{t,j}$ means the attention scores computed on the tokens generated by the sampled approach. Our theorem assumes that dropping the tokens depends on the attention score of the current iteration. This assumption is close to our algorithm, where we drop tokens based on attention scores in previous iterations, since in Section \ref{sec:hypos} we argued both theoretically and through experiment that the large attention scores will remain large through the whole generation process.

(\ref{eq:err_bound}) provided a bound on the expected difference between the tokens generated in the sampled and unsampled approach. Observe that the upper bound scales with $1-B$, and when $B$ is $1$, meaning that we are keeping all of the tokens, the error becomes zero. The term $\paren{k -  (k-1)\paren{\frac{1-\epsilon}{B-\epsilon}}^{\frac{1}{k-1}}}$ depends on the distribution that the attention scores are fitted to and is always less than one. With a nicely chosen power-law distribution, this term provides a further decrease to the error bound in (\ref{eq:err_bound}).
%\input{B_algorithm}

\ww{I will try to add another proof to show that the selection of tokens or the sampling of tokens is optimal under the constraints of cache sizes. Please feel free to formalize my proof.}

\ww{The sampling and token generation system is actually a chaos system, thus its performance is unpredictable across different sequence lengths, different cache sizes, and different datasets. To prove something out of this system, we need to add additional assumptions according to the experimental results.}

From the observation of Figure~\ref{}, the token score generated from the sampled KV cache is almost the same as the original KV cache, which also echoes Theorem~\ref{theo:error_bound}. 

With this assumption that the attention scores in \name{} are almost the same as the original inference, the problem has been reformulated as picking a number of tokens that can fit into the cache size and achieving the most similar performance as the original KV cache.

Denote the maximum number of tokens that can be stored in the cache is $B$. With the sampling strategy in \ref{sec:method_sample}, the tokens with the highest scores will usually be preserved in the cache. Denote the $B$ number of tokens with the highest score as $\{x^{topB}_t\}_{t=0}^T$. 

For any other sets of tokens $\{x'_t\}_{t=0}^T$ that has no greater than $B$ number of tokens in the cache, we can easily prove that:

\begin{equation}
    similarity\left(x^{topB}_t, x_t\right) \leq \left(x'_t, x_t\right)
\label{equ:optimal}
\end{equation}

The actual proof can be given with an induction: 1) when $t \le c$, all tokens will be kept, so $\{\tilde{x}_t\}_{t=0}^c = \{\tilde{x}'_t\}_{t=0}^c = \{x_t\}_{t=0}^c$; when $t > c$, use induction to prove Equation~\ref{equ:optimal}.

\ww{My two cents is that, when the cache size keeps decreasing, the bound may be hard to find, but the expected performance of our sampling method may be proved to be optimal.}

==> A01_related.tex <==

% \section{Related Work}
% \noindent \textbf{Quantization, pruning, distillation for LLM inference.} Various system relaxations have been studied for decades for model inference in machine learning. For example, quantization~\cite{han2015deep, jacob2018quantization,nagel2019data,zhao2019improving}, pruning~\cite{molchanov2016pruning,liu2018rethinking,he2019filter,hoefler2021sparsity}, and distillation~\cite{hinton2015distilling,cho2019efficacy,tang2019distilling,touvron2021training}  have been applied to speed up the inference of the machine learning model. Active research has recently attempted to apply such techniques in LLM inference. For example, zeroQuant~\cite{yao2022zeroquant} and nuQmm~\cite{park2022nuqmm} implement customized CUDA kernels to support tenor-wise or group-wise quantization for LLM inference; LLM.int8 \cite{dettmers2022llm} adopts a mixed \texttt{INT8/FP16} computation to diminish the influence of activation outliers; SmoothQuant~\cite{xiao2022smoothquant} enables efficient 8-bit weight and activation for LLM inference; GPTQ~\cite{frantar2022gptq} adopts a one-shot weight quantization method based on approximate second-order information for accuracy and efficiency; SparseGPT~\cite{frantar2023massive} introduces an approximate sparse regression solver to enable the sparsity in LLM inference; \cite{bansal2022rethinking} has reported that a small set of attention heads can perform primitive induction operations associated with in-context learning, and use this property to prune LLM for acceleration. 

==> A02_theory.tex <==
\section{Overall story}
{ \color{ashgrey}
The problem of sampling and quantizing kv-cache can naturally cast as approximating the output of attentions. We can analyse quantization and sampling separately. A note on sampling : Given the nature of sampling, a closely related problem is that of reservoir sampling. However, the problem is slightly different as the weights associated with the weighted summation change with addition of new tokens which opens up new avenues for variance reduction. We start with simple abstract sampling design with E(S)=1.

1. Any sampling design that ensures $E(S_i) = 1$ is a good to get almost unbiased estimates of attention

2. Variance reduction of denominator ( also numerator)  requires sampling with probability proportional to weights.  While the problem of weighted reservoir sampling is well understood, the problem of dynamic weights is rather understudied (verify) and often ifeasible. 

3. We give a reservior sampling for dynamic weights with weight evolution assumptions motivated from the problem at hand. ($ \pi(k|j) < \pi(k|j-1)$.  The algorithm and proof are straightfroward. 

4. Proving / intuiton as to why the assumption holds. Either jaspers proof can be modified for this or can be used as a intuition.  Also, we can give empirical evidence. 

We can thus cover the sampling part under standard (modifed) sampling theory and the sections can be made rigorous with notations borrowed from the sampling literature.

Quantisation can be analysed separately. Although it deviates from the central story

In this section we will talk about reduction of kv-cache for a particular attention head given a budget of tokens say $n$. The problem can be interpreted as sampling problem with the target to get an accurate estimate of the output of attention head at token, say $t+1$. The computation in attention can be written as,

\begin{align*}
    a_{t+1} = W_V X_{t-1} \textrm{ softmax } (X_{t-1}^\top W_{KQ} x_t) \\
    a_{t+1} = \sum_{j=1}^{t-1} \frac{\exp(\langle k_j, q_t \rangle ) v_j}{ \sum_{j=1}^{t-1} \exp(\langle k_j , q_t)} \\
    a_{t+1} = \frac{ \sum_{j=1}^{t-1} \exp(\langle k_j, q_t \rangle ) v_j}{ \sum_{j=1}^{t-1} \exp(\langle k_j , q_t)}
\end{align*}
where $q_j = x_j W_Q $,   $k_j = x_j W_K $ and $v_j = x_j W_V $

Let $\rho(j ; t ) = \exp(k_j, t)$, then we can write the attention output as,
\begin{align*}
    a_{t+1} = \frac{ \sum_{j=1}^{t-1} \rho(j ; t) v_j}{ \sum_{j=1}^{t-1} \rho(j; t)}
\end{align*}

Let $S$ be the random variable denoting sample chosen. It is important to note that if we estimate the quantity above by, 
\begin{align*}
    X = \frac{ \sum_{j=1}^{t-1} S_i \frac{\alpha_i}{p_i} \rho(j ; t) v_j}{ \sum_{j=1}^{t-1} S_i \rho(j; t)}
\end{align*}

where $\alpha_j = \frac{\rho(j;t) }{\sum_j \rho(j ; t) }$
The above estimator works for any sampling design with single sized samples. But if we sample with a distribution different from $\alpha_i$, we need to know the values of $\alpha_j$ for sampled $j$ which requires exact computation of the partition function (denominator).

Can the same estimator work for sample size $n$ designs? Lets consider $n=2$

\begin{align*}
    E(X) = \frac{1}{^{(t-1)}C_2} \sum_{i,j} \left( \frac{\frac{(t-1)\alpha_i}{2} \rho_i +  \frac{(t-1)\alpha_j}{2} \rho_j}{\rho_i + \rho_j}\right)
\end{align*}

This is not unbiased. Seems like writing an unbiased estimator with just inclusion properties as the statistic is not possible in this case {\color{red} can we prove this negative?} . In such a case, we can bound the bias if we can talk about strong estimation guarantee of the denominator.

If we assume that $\sum_{j=1}^{(t-1)} \frac{S_i}{p_i} \rho(j;t) = (1 \pm \epsilon)  \sum_{j=1}^{(t-1)} \rho(j;t)$ with probability $(1- \delta)$ where $\delta$ is very small, we can make a statement about bias of the following estimator 

where 
\begin{align*}
    X_l = (1 - \epsilon) \frac{ \sum_{j=1}^{t-1} \frac{S_i}{p_i} \rho(j ; t) v_j}{ \sum_{j=1}^{t-1} \rho(j; t)} \qquad X_r = (1 + \epsilon) \frac{ \sum_{j=1}^{t-1} \frac{S_i}{p_i} \rho(j ; t) v_j}{ \sum_{j=1}^{t-1} \rho(j; t)}
\end{align*}

In discrete case,  (change of notation)
\begin{equation}
    E(X) = (p_1 x_1 + .......p_k x_k) + (p_{k+1} x_{k+1} +  ... p_n x_n)
\end{equation}
\begin{equation}
    E(X_r) = (p_1 r_1 + .......p_k r_k) + (p_{k+1} r_{k+1} +  ... p_n r_n)
\end{equation}

and $(p_{k+1} + ... p_n) < \delta $

\begin{align*}
    E(X_l) - \delta \max_S(X_l - X) \leq E(X) \leq  E(X_r) + \delta \max_S(X - X_r) \\
    |Bias(X)| \leq \epsilon a_{t+1} + \delta (\max_S(\max(X - X_r, X_l - X)))
\end{align*}



With a power law assumption on $\rho$ we can potentially get rid of $\delta$? and have $\epsilon$ in terms of power-law coefficient and sample size. 
\begin{equation}
    (1 - \epsilon) a_{t+1} \leq E(X) \leq  (1+\epsilon) a_{t+1} \qquad  ; \qquad    |Bias(X)| \leq \epsilon a_{t+1}
\end{equation}
}


We will use the following estimator , 
\begin{align*}
    \hat{b} = \frac{\sum \frac{S_i}{\pi_s[i]} w_i \bar{v}_i}{\sum w_i}
\end{align*}
\begin{align*}
    \hat{a} = \frac{\sum \frac{S_i}{\pi_s[i]} w_i \bar{v}_i}{\sum \frac{S_i}{\pi_s[i]}w_i}
\end{align*}
\begin{align*}
    \hat{a} = \hat{b} \frac{1}{\sum \frac{S_i}{\pi_s[i]} \alpha_i}
\end{align*}

\section{Reservoir sampling } \label{appendix:sampling}

\textbf{Approach}

\textbf{Sampling design:} Based on the above observations, we propose the following sampling design. Let $\pi(t;i)$ be the first-order probability of inclusion of token $i \leq t$ at $(t+1)$ token generation step. We propose a sampling design parameterized by budget $n$ and recent window size $r$,
\begin{equation}
    \pi(t, i) \begin{cases}
    = 1  & \textrm{ if } i > t - r \\
    \propto Z_{ti} = \max\left( \left\{ \frac{\rho(t-j, i)}{\sum_{k=1}^{t-j} \rho(t-j, k) } \right\}_{j=0}^{r-1}\right)  & \textrm{ otherwise }
    \end{cases}
\end{equation}
We aim to keep a recent history of $r$ tokens in our sample, Other tokens such as those previously generated and those from the prompt are included with probability proportional to their maximum contribution to recent $r$ tokens (i.e. $Z_{ti}$). We assume that $n > r + p$. We first set all the inclusion probabilities of recent tokens to $1$. For the rest, we compute inclusion probabilities in accordance with Chao's procedure \cite{chao1982general} with $Z_{ti}$ as the weights and $(n - r)$ as the budget. We can summarize the process as follows,

\begin{itemize}
    \item if $n \geq t$, then all the $\pi(t,i) = 1$
    \item if $n < t$, then 
    \begin{itemize}
        \item if $(t - i ) < r$, then $\pi(t, i) = 1$ 
        \item if $(t - i ) \geq r$, then we compute $\frac{(n - r) Z_{ti}}{\sum_{i=1}^t Z_{ti}}$. If this value for some $i$ is greater than $1$ we set the inclusion probability of the token with highest value as $1$ and recursively repeat the process with $(n-r-1)$ budget for remaining tokens till all values are less than 1. We then set all the inclusion probabilities equal to the values computed.
    \end{itemize}
\end{itemize}

The inclusion probabilities set above satisfy,
\begin{equation}
    \sum_{i=1}^t \pi(t; i) = n ; \qquad 0 < \pi(t; i) <= 1
\end{equation}

The reservoir sampling procedure is presented in algorithm \ref{alg:sampling}
\input{algorithms/sampling}. Our procedure maintains the sample at $t$ with inclusion probabilities equal to $\min_{j \in \{1, ...., t\}}(\pi(j, i))$. 

\textbf{Computing attention output:}
At generation of token $t$, let S be the binary vector of size $t-1$ denoting the sample maintained in the reservoir. Also, let $\pi_s$ be the probability of sample as computed in algorithm \ref{alg:sampling}. We use the following estimator to compute the attention output

\begin{align}
    \hat{a}_t = \frac{\sum_{i=1}^t \frac{S[i]}{\pi_s[i]} \rho(t, i) (W_V x_i)}{ \sum_{i=1}^t \frac{S[i]}{\pi_s[i]} \rho(t, i)}
\end{align}




==> algorithms/sampling.tex <==
\begin{algorithm}
\caption{Reservoir sampling of tokens to keep in kv cache with budget $n$} \label{alg:sampling}
\begin{algorithmic}
\Require $n \geq 0$, $x_t$ : embedding at next token at $t$,  Sample $S$ of tokens maintained till now. Inclusion probabilities at previous and new tokens $\pi(t-1, i)$ and $\pi(t, i)$.

\Ensure $S$ is updated to respect the inclusion probabilities $\pi(t, i)$ and budget $|S| \leq n$

\If{$t \leq n $}
    \State $S = S \cup \{ t \}$
    \State $\pi_{s}[t] = 1$
\ElsIf{ $t > n$}
    \State Select a token $k$ from the sample $S$ with probabilities 
    \begin{equation}
        \left[1 - \max \left( 1, \frac{\pi(t, k)}{\pi_{s}[k]} \right) \right]
    \end{equation}
    \If{$\pi(t, k) < \pi_{s}[k]$}
        \State $\pi_{s}[k] = \pi(t, k)$
    \EndIf
    \State $S = S / \{k\} \cup \{t\}$
\EndIf

\end{algorithmic}
\end{algorithm}

==> algorithms/sampling_1.tex <==
\begin{algorithm}
\caption{Sampling of tokens to keep in KV cache with budget $N$} \label{alg:sampling}
\begin{algorithmic}
\Require $N \geq 0$, $x_t$ : embedding at next token at $t$,  Sample $S_{t-1}$ of tokens maintained till now. Recency window $r$

\Ensure return $S_t$, $\{ t{-}r{+}1, ..., t \} \subset S_t$,  $|S| \leq N$

\If{$t \leq N $}
    \State $S_t = S_{t-1} \cup \{ t \}$
\ElsIf{ $t > N$ }
    \State  For $s$ in $\{t{-}r{+}1, ..., t\}$
    \State $$\pi(t, s) = 1$$  
    \State For $s \in S/\{t{-}r{+}1, ..., t{-1}\}$
    \State $$Z_{ts} = \max \left(  \left\{  \alpha_{t-j,i} \right\}_{j=1}^r \right)$$ 
    \State 
    \begin{equation}
        \pi(t, s) = \textrm{ Inclusion probability proportional to } Z_{ts} \textrm{with size } (n-r) \textrm{(IPPS)\cite{tille2006sampling}}
    \end{equation}
    \State Select a token $k$ from the sample $S$ with probabilities $\left(1 - \pi(t, k) \right)$
    \State $S_t = S_{t-1} / \{k\} \cup \{t\}$
\EndIf

\end{algorithmic}
\end{algorithm}
